Prospective Learning: Principled Extrapolation to the Future

Learning is a process which can update decision rules, based on past experience, such that future performance improves. Traditionally, machine learning is often evaluated under the assumption that the future will be identical to the past in distribution or change adversarially. But these assumptions can be either too optimistic or pessimistic for many problems in the real world. Real world scenarios evolve over multiple spatiotemporal scales with partially predictable dynamics. Here we reformulate the learning problem to one that centers around this idea of dynamic futures that are partially learnable. We conjecture that certain sequences of tasks are not retrospectively learnable (in which the data distribution is fixed), but are prospectively learnable (in which distributions may be dynamic), suggesting that prospective learning is more difficult in kind than retrospective learning. We argue that prospective learning more accurately characterizes many real world problems that (1) currently stymie existing artificial intelligence solutions and/or (2) lack adequate explanations for how natural intelligences solve them. Thus, studying prospective learning will lead to deeper insights and solutions to currently vexing challenges in both natural and artificial intelligences.

==> backmatter/diversity.tex <==
% Updated on 8/08/2022
\section*{References Diversity Statement}
By our estimates (using \href{https://github.com/dalejn/cleanBib}{cleanBib}), 
our references contain 11.47\% woman(first)/woman(last), 22.06\% man/woman, 22.06\% woman/man, and 44.41\% man/man, and 
11.11\% author of color (first)/author of color(last), 13.84\% white author/author of color, 14.88\% author of color/white author, and 60.17\% white author/white author.

==> backmatter/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm,dsfont}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% Reference to an equation, lower-case.
\def\ineqref#1{Inequality~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}
% Reference to a definition, lower case
\def\defref#1{Definition~\ref{#1}}
% Reference to a remark, lower case
\def\remref#1{Remark~\ref{#1}}
% Reference to a conjecture, lower case
\def\conref#1{Conjecture~\ref{#1}}

\def\ceil#1{\lceil #1 \rceil}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}


\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\providecommand{\mc}[1]{\mathcal{#1}}
\providecommand{\mh}[1]{\hat{#1}}

% \newtheorem{definition}{Definition}
% \newtheorem{remark}{Remark}
% \newtheorem{conjecture}{Conjecture}


==> frontmatter/nd_preamble.tex <==
%===============================================================================%
% This is the neurodata latex preamble.
%
% We have desigend it to augment the SIAM LaTeX2e Multimedia Macros for
% Online-Only Journals, located here:
% https://www.siam.org/Portals/0/Macros/Online/siamonline_190516.zip
%
% If you need a specific package please load it here.
%===============================================================================%

\usepackage{comment}
\usepackage{lipsum}
\usepackage[margin=1in, footskip=36pt]{geometry}

% fontspec commented out due to rendering issue observable in prospective learning overleaf; this breaks Eric's pretty table
% \usepackage{fontspec}

% \usepackage{array,colortbl,pifont}
%%% For author, thanks, affil
%\usepackage[noblocks]{authblk}
\usepackage{endnotes}
\renewcommand{\notesname}{Affiliations}

% loading TOC class from outside of SIAM
% this has to be followed by reconfig of a series commands in the associated cls file
\usepackage{tocloft}

\renewcommand{\contentsname}{Table of Contents}
% \usepackage{titletoc}
% \usepackage{tocbasic}

\usepackage{titlesec}
\usepackage{titletoc}
\usepackage{pgfplotstable}

\definecolor{darktangerine}{rgb}{1.0, 0.77, 0.07}
\definecolor{aogr}{rgb}{0.0, 0.5, 0.0}

%% Set Up Checks/Xs

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\boldq}{\textbf{?}}

\newcommand{\greencheck}{\textcolor{aogr}\cmark}
\newcommand{\ocheck}{\textcolor{darktangerine}\cmark}
\newcommand{\yellowq}{\textcolor{darktangerine}\boldq}
\newcommand{\redx}{\textcolor{red}\xmark}

%%=================
%% Define Headings and section task
%%=================
\titleclass{\task}{straight}[\section]
\newcounter{task}
\renewcommand{\thetask}{\arabic{task}}
\titleformat{\task}[hang]
    {\normalfont\LARGE\bfseries}{Task \thetask:}{1em}{}


\titleformat*{\task}{\color{header1}\bfseries}

\titlecontents{task}
              [3.8em] % ie, 1.5em (chapter) + 2.3em
              {}
              {\contentslabel{2.3em}}
              {\hspace*{-2.3em}}
              {\titlerule*[1pc]{.}\contentspage}


\titlespacing*{\section}{0ex}{1ex}{1ex}
\titlespacing*{\subsection}{0ex}{1ex}{1ex}
\titlespacing*{\subsubsection}{0ex}{1ex}{1ex}
\titlespacing*{\paragraph}{0ex}{1ex}{1ex}
\titlespacing*{\subparagraph}{0pt}{1ex}{1ex}
\titlespacing*{\task}{0em}{1ex}{1ex}


%%% for footnote affiliation block
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

%%% Bib and citations
\usepackage[sort&compress,comma,square,numbers]{natbib}

%%% mathfonts, equation environments and eqref, ...
\usepackage{amsfonts,amsmath,amssymb}
\usepackage{bbm}

%%% For enumitem with special global options
\usepackage{multicol}
\usepackage{enumitem}
\setlist[enumerate]{wide, labelindent=1cm,  noitemsep}
% \setlist[enumerate]{noitemsep}
\setlist[itemize]{noitemsep}
\setlist[description]{noitemsep}

%%% For colors and sout and hhlines
\usepackage{hhline}
\definecolor{MSBlue}{rgb}{.204,.353,.541}
\definecolor{slate}{rgb}{0.156,0.184,0.180}
\definecolor{lgray}{rgb}{0.312,0.368,0.360}
\definecolor{vlgray}{rgb}{0.95, 0.95, 0.95}

%%%%%%%%%%% EDITING MACROS %%%%%%%%%%%%%
\usepackage{todonotes}
\RequirePackage{ulem}
\newcommand{\add}[1]{\textcolor{blue}{[#1]}}
\newcommand{\rep}[2]{\textcolor{brown}{[\sout{#1} $|$ #2]}}
\newcommand{\dele}[1]{\textcolor{red}{\sout{#1}}}

%% Set up Tables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%===%
\definecolor{tableheadcolor}{gray}{0.92}
% Following is taken from Werner: http://tex.stackexchange.com/a/33761/3061
% and modified for my needs
%
% Command \topline consists of a (slightly modified)
% \toprule followed by a \heavyrule rule of colour tableheadcolor
% (hence, 2 separate rules)
\newcommand{\topline}{ %
        \arrayrulecolor{blue1}\specialrule{0.1em}{\abovetopsep}{0pt}%
        \arrayrulecolor{tableheadcolor}\specialrule{\belowrulesep}{0pt}{0pt}%
        \arrayrulecolor{blue1}}
% Command \midline consists of 3 rules (top colour tableheadcolor, middle colour black, bottom colour white)
\newcommand{\midtopline}{ %
        \arrayrulecolor{tableheadcolor}\specialrule{\aboverulesep}{0pt}{0pt}%
        \arrayrulecolor{blue1}\specialrule{\lightrulewidth}{0pt}{0pt}%
        \arrayrulecolor{white}\specialrule{\belowrulesep}{0pt}{0pt}%
        \arrayrulecolor{blue1}}
% Command \bottomline consists of 2 rules (top colour
\newcommand{\bottomline}{ %
        \arrayrulecolor{white}\specialrule{\aboverulesep}{0pt}{0pt}%
        \arrayrulecolor{blue1} %
        \specialrule{\heavyrulewidth}{0pt}{\belowbottomsep}}%


\newcommand{\midheader}[2]{%
        \midrule\topmidheader{#1}{#2}}
\newcommand\topmidheader[2]{\multicolumn{#1}{c}{\textsc{#2}}\\%
                \addlinespace[0.5ex]}

\pgfplotstableset{normal/.style ={%
        header=true,
        string type,
        font=\small,
    	column type={p{.092\textwidth}},
        every head row/.style={
            before row={\topline\rowcolor{tableheadcolor}},
            after row={\midtopline}
        },
        every odd row/.style={
            before row={\rowcolor{blue1}}
        },
        every last row/.style={
            after row=\bottomline
        },
        col sep=&,
        row sep=\midrule
    }
}

\usepackage{multirow}


%%% for \toprule
\usepackage{booktabs}
\usepackage{fancyhdr}
\usepackage{fullpage}

% Define LaTeX friendly Fonts
%==============
\RequirePackage{titlesec}
\RequirePackage[font={footnotesize},{singlelinecheck=false}]{caption}
\captionsetup{belowskip=-5pt}

\usepackage[T1]{fontenc}
\usepackage[scaled]{helvet}
\usepackage[scaled=1.10, med]{zlmtt}
\renewcommand\familydefault{\sfdefault}


%%% For begin{algorithm}
\usepackage{algorithm}
\usepackage{algpseudocode}

\newcommand{\Linefor}[2]{%
    \State \algorithmicfor\ {#1}\ \algorithmicdo\ {#2} \algorithmicend\ \algorithmicfor%
}
\newcommand{\Lineif}[2]{%
    \State \algorithmicif\ {#1}\ \algorithmicdo\ {#2} \algorithmicend\ \algorithmicif%
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% MACROS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%% ALGORITHM NAMES %%%%%%%%%%%%%
\providecommand{\sct}[1]{{\sc \texttt{#1}}}

\newcommand{\Idt}{\sct{Idt}}
\newcommand{\Svd}{\sct{Svd}}
\newcommand{\Pca}{\sct{Pca}}
\newcommand{\Fld}{\sct{Fld}}
\newcommand{\Lda}{\sct{Lda}}
\newcommand{\eig}{\sct{eig}}
\newcommand{\Lol}{\sct{Lol}}
\newcommand{\Lal}{\sct{Lal}}
\newcommand{\Qoq}{\sct{Qoq}}
\newcommand{\Lrl}{\sct{Lrl}}
\newcommand{\Lfl}{\sct{Lfl}}
\newcommand{\Faq}{\sct{Faq}}
\newcommand{\qr}{\sct{qr}}

\newcommand{\Mgc}{\sct{Mgc}}
\newcommand{\Mgcp}{\Mgc$_P$}
\newcommand{\Mgcd}{\Mgc$_D$}
\newcommand{\Mgcm}{\Mgc$_M$}
\newcommand{\Hhg}{\sct{Hhg}}
\newcommand{\Dcorr}{\sct{Dcorr}}
\newcommand{\Dcov}{\sct{Dcov}}
\newcommand{\Mcorr}{\sct{Mcorr}}
\newcommand{\Mantel}{\sct{Mantel}}
\newcommand{\Mic}{\sct{Mic}}
\newcommand{\Hsic}{\sct{Hsic}}
\newcommand{\Pearson}{\sct{Pearson}}
\newcommand{\Kendall}{\sct{Kendall}}
\newcommand{\Spearman}{\sct{Spearman}}
\newcommand{\RV}{\sct{RV}}
\newcommand{\CCA}{\sct{Cca}}
\newcommand{\Sporf}{\sct{Sporf}}
\newcommand{\Mf}{\sct{Mf}}
\newcommand{\MF}{\sct{RF}}
\newcommand{\ICC}{\sct{ICC}}



%%%%%%% MATH OPERATORS %%%%%%%%%%%%

\providecommand{\ve}[1]{\boldsymbol{#1}}
\providecommand{\ma}[1]{\boldsymbol{#1}}
\providecommand{\deter}[1]{\lvert #1 \rvert}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argsup}{\operatornamewithlimits{argsup}}
\newcommand{\arginf}{\operatornamewithlimits{arginf}}
\newcommand{\T}{^{\ensuremath{\mathsf{T}}}} % transpose
\providecommand{\norm}[1]{\ensuremath{\left \lVert#1 \right  \rVert}}
\providecommand{\abs}[1]{\ensuremath{\left \lvert #1 \right \rvert}}
% \providecommand{\mat}[1]{\left[ #1 \right]}
% \newcommand{\trans}[1]{{#1}^{\ensuremath{\mathsf{T}}}}    % \newcommand{\transpose}[1]{{#1}^{\ensuremath{\mathsf{T}}}}
\newcommand{\from}{{\ensuremath{\colon}}}           % :
\newcommand{\trace}[1]{{\ensuremath{\operatorname{tr}\!\left(#1\right)}}}           % :
%
\providecommand{\mc}[1]{\mathcal{#1}}
\providecommand{\tmc}[1]{\tilde{\mathcal{#1}}}
\providecommand{\mb}[1]{\boldsymbol{#1}}
\providecommand{\ms}[1]{\mathsf{#1}}
\providecommand{\mt}[1]{\widetilde{#1}}
\providecommand{\mbb}[1]{\mathbb{#1}}
\providecommand{\mv}[1]{\vec{#1}}
\providecommand{\mh}[1]{\hat{#1}}
\providecommand{\wh}[1]{\widehat{#1}}
\providecommand{\mhv}[1]{\mh{\mv{#1}}}
\providecommand{\mvh}[1]{\mv{\mh{#1}}}
\providecommand{\mhc}[1]{\hat{\mathcal{#1}}}
\providecommand{\mbc}[1]{\mb{\mathcal{#1}}}
\providecommand{\mvc}[1]{\mv{\mathcal{#1}}}
\providecommand{\mtc}[1]{\widetilde{\mathcal{#1}}}
\providecommand{\mth}[1]{\mt{\mh{#1}}}
\providecommand{\mht}[1]{\mh{\mt{#1}}}
\providecommand{\mhb}[1]{\hat{\boldsymbol{#1}}}
\providecommand{\whb}[1]{\widehat{\boldsymbol{#1}}}
\providecommand{\mvb}[1]{\vec{\boldsymbol{#1}}}
\providecommand{\mtb}[1]{\widetilde{\boldsymbol{#1}}}
\providecommand{\mbt}[1]{\widetilde{\boldsymbol{#1}}}
\providecommand{\mvc}[1]{\vec{\mathcal{#1}}}
% \newcommand{\D}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dd}[2]{\frac{\partial ^2 #1}{\partial #2 ^2}}
\newcommand{\DDD}[3]{\frac{\partial ^2 #1}{\partial #2 \partial #3}}
\newcommand{\Di}[2]{\frac{\partial ^i #1}{\partial #2 ^i}}



%%%%%%%%% SHORT HAND %%%%%%%%%%
\newcommand{\website}{\url{https://neurodata.io/}}
\newcommand{\jhu}{Johns Hopkins University}
\newcommand{\jvemail}{\href{mailto:jovo@jhu.edu}{jovo@jhu.edu}}
\newcommand{\jv}{Joshua T.~Vogelstein}

\newcommand{\Vr}{V_{reset}}
\newcommand{\Vl}{V_{leat}}
\newcommand{\eqdef}{\overset{\triangle}{=}}
\newcommand{\grad}{\nabla}
\newcommand{\Hess}{\nabla\nabla}
\newcommand{\defn}{\overset{\triangle}{=}}

\newcommand{\rto}{\leftarrow}
\newcommand{\iid}{\overset{iid}{\sim}}
\newcommand{\knn}{$k$NN}

\newcommand{\elegans}{\emph{C. elegans} }

\newcommand{\Lik}{\mathcal{L}}
\newcommand{\Cae}{[\widehat{\text{Ca}}^{2+}]}
\newcommand{\Cav}{\ve{C}}%[\ve{\text{Ca}}^{2+}]}
\newcommand{\sml}{\sqrt{\ma{\lambda}}}
\newcommand{\ml}{\ma{\lambda}}
\newcommand{\nw}{\widehat{n}}
\newcommand{\nv}{\vec{n}}
\newcommand{\Ae}{\widehat{A}}
\newcommand{\te}{\widehat{\tau}}
\newcommand{\maxn}{\max_{\ve{n}: n_t \geq 0}}
% \newcommand{\V}{\text{Var}}

\newcommand{\PmcP}{P \in \mc{P}}
\newcommand{\mP}{\mathbb{P}}

% \newcommand{\dvs}{\dot{\bs}_t}
% \newcommand{\dvw}{\dot{\bw}_t}
% \newcommand{\dvx}{\dot{\bx}_t}
% \newcommand{\dvy}{\dot{\by}_t}

\newcommand{\ft}{f_{\ve{\thet}}}
\newcommand{\gt}{g_{\ve{\thet}}}
\newcommand{\hht}{h_{\thetn}}

\newcommand{\Real}{\mathbb{R}}
\newcommand{\Ind}{\mathbb{I}}

\newcommand{\wconv}{\overset{i.p.}{\rightarrow}}
\newcommand{\sconv}{\overset{i.p.}{\rightarrow}}
\newcommand{\conv}{\rightarrow}
\newcommand{\pconv}{\overset{p}{\conv}}
\newcommand{\mcE}{\mathcal{E}}
\newcommand{\mcT}{\mathcal{T}}
\newcommand{\mcG}{\mathcal{G}}
\newcommand{\mcM}{\mathcal{M}}
\newcommand{\mcL}{\mathcal{L}}
\newcommand{\hatmcE}{\widehat{\mcE}}
\newcommand{\hatp}{\widehat{p}}
\newcommand{\hatP}{\widehat{P}}
\newcommand{\hatQ}{\widehat{Q}}
\newcommand{\hatL}{\widehat{L}}
\newcommand{\mhP}{\widehat{\PP}}
\newcommand{\tildeA}{\widetilde{A}}
\newcommand{\defeq}{\overset{\triangle}{=}}


\DeclareMathOperator{\Pmat}{\mathbf{P}}
\DeclareMathOperator{\veta}{\mathbf{\mb{v}}}
\DeclareMathOperator*{\minimize}{\mathrm{minimize}}
\DeclareMathOperator*{\maximize}{\mathrm{maximize}}
% \DeclareMathOperator*{\mb{v}mod}{\mathbf{\mb{v}}}


%%%%%%% LATIN LETTERS


\newcommand{\bA}{\mb{A}}
\newcommand{\bB}{\mb{B}}
\newcommand{\bD}{\mb{D}}
\newcommand{\bE}{\mb{E}}
\newcommand{\bI}{\mb{I}}
\newcommand{\bP}{\mb{P}}
\newcommand{\bS}{\mb{S}}
\newcommand{\bU}{\mb{U}}
\newcommand{\bV}{\mb{V}}
\newcommand{\bW}{\mb{W}}
\newcommand{\bX}{\mb{X}}
\newcommand{\bY}{\mb{Y}}
\newcommand{\bZ}{\mb{Z}}

\newcommand{\ba}{\mb{a}}
\renewcommand{\ba}{\mb{b}}
\newcommand{\bd}{\mb{d}}
\newcommand{\be}{\mb{e}}
\newcommand{\bp}{\mb{p}}
\newcommand{\bs}{\mb{s}}
\newcommand{\bu}{\mb{u}}
\newcommand{\bv}{\mb{v}}
\newcommand{\bw}{\mb{w}}
\newcommand{\bx}{\mb{x}}
\newcommand{\by}{\mb{y}}
\newcommand{\bz}{\mb{z}}


\newcommand{\Aa}{\mathbb{A}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\EE}{\mathbb{E}}           % expected value
\newcommand{\FF}{\mathbb{F}}
\newcommand{\GG}{c}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}           % indicator function
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}}




\newcommand{\Qs}{Q}
\newcommand{\mcS}{\mc{S}}
\newcommand{\mcU}{\mc{U}}

\newcommand{\mbd}{\ensuremath{\mb{d}}}
\newcommand{\mbD}{\ensuremath{\mb{D}}}
\newcommand{\mbx}{\ensuremath{X}}
\newcommand{\mbX}{\ensuremath{\mb{X}}}
\newcommand{\mby}{\ensuremath{Y}}
\newcommand{\mbY}{\ensuremath{\mb{Y}}}

\newcommand{\mtbd}{\mtb{d}}
\newcommand{\mtbD}{\mtb{D}}
\newcommand{\mtbx}{\mtb{x}}
\newcommand{\mtbX}{\mtb{X}}
\newcommand{\mtby}{\mtb{y}}
\newcommand{\mtbY}{\mtb{Y}}



\DeclareMathOperator{\Ri}{\mathbf{\R}^{-1}}
\DeclareMathOperator{\A}{A}
\DeclareMathOperator{\W}{\mathbf{W}}
\DeclareMathOperator{\V}{\mathbf{V}}
%\DeclareMathOperator{\U}{\mathbf{U}}
%\DeclareMathOperator{\C}{\mathbf{C}}
\DeclareMathOperator{\uvec}{\mathbf{u}}
\DeclareMathOperator{\D}{\mathbf{D}}
\DeclareMathOperator{\Q}{\mathbf{Q}}
\DeclareMathOperator{\R}{R} %\mathbf{P}}
\DeclareMathOperator{\Y}{\mathbf{Y}}
%\DeclareMathOperator{\BB}{\mathbf{B}}
\DeclareMathOperator{\Hmat}{\mathbf{H}}
\DeclareMathOperator{\Gmat}{\mathbf{G}}
\DeclareMathOperator{\X}{\mathbf{X}}
\DeclareMathOperator{\Cmat}{C} %\mathbf{L}}\providecommand{\ms}[1]{\mathsf{#1}}

\DeclareMathOperator*{\Ymod}{\mathbf{\Y}}
\DeclareMathOperator*{\Bmod}{\mathbf{B}}
\DeclareMathOperator*{\Hmod}{\mathbf{H}}
\DeclareMathOperator*{\Lmod}{\mathbf{L}}
\DeclareMathOperator*{\Xmod}{\mathbf{\X}}


%%% THETA %%%%

\newcommand{\bth}{\ve{\theta}}
\newcommand{\hth}{\mh{\theta}}
\newcommand{\htth}{\mh{\theta}}
\newcommand{\bhth}{\mh{\ve{\theta}}}
\newcommand{\thetn}{\ve{\theta}}
\newcommand{\thet}{\thetn}
\newcommand{\theth}{\widehat{\ve{\theta}}}
\newcommand{\theto}{\ve{\theta}'}
\newcommand{\wht}{\widehat{\thet}}
\newcommand{\wtt}{\widetilde{\thet}}
\newcommand{\vth}{\ve{\thet}}
\newcommand{\vTh}{\ve{\Theta}}
\newcommand{\hvth}{\widehat{\ve{\thet}}}
\newcommand{\bTh}{\ve{\Theta}}
\newcommand{\hbth}{\widehat{\thet}}
\newcommand{\tbth}{\tilde{\bth}}



% \newcommand{\p}{P_{\bth}}
\newcommand{\pold}{P_{\bth'}}
\newcommand{\pk}{P_{\widehat{\ve{\theta}}^{(k)}}}
\newcommand{\pT}{P_{\thetn_{Tr}}} %\thetn_T
\newcommand{\pO}{P_{\thetn_o}} %\thetn_o
% \newcommand{\Q}{Q(\thetn,\theto)}
% \newcommand{\m}{m^{\ast}}
% \newcommand{\q}{q(\ve{H}_t)}
\newcommand{\Ca}{[\text{Ca}^{2+}]}


%%%%%% GREEK LETTERS

\newcommand{\del}{\delta}
\newcommand{\sig}{\sigma}
\newcommand{\lam}{\lambda}
\newcommand{\gam}{\gamma}
\newcommand{\eps}{\varepsilon}

\newcommand{\Del}{\Delta}
\newcommand{\Sig}{\Sigma}
\newcommand{\Lam}{\Lambda}
%\newcommand{\Gam}{\Gamma}

\newcommand{\bSig}{\ve{\Sigma}}
\newcommand{\bOm}{\ve{\Omega}}
\newcommand{\bLam}{\ve{\Lambda}}
\newcommand{\bPhi}{\ve{\Phi}}
\newcommand{\bPsi}{\ve{\Psi}}

\newcommand{\bmu}{\ve{\mu}}
\newcommand{\bal}{\ve{\alpha}}
\newcommand{\bpi}{\ve{\pi}}
\newcommand{\bkap}{\ve{\kappa}}
\newcommand{\bdel}{\ve{\delta}}
\newcommand{\bphi}{\ve{\phi}}
\newcommand{\bpsi}{\ve{\psi}}



\DeclareMathOperator{\Delti}{\mathbf{\Delta}^{-1}}
\DeclareMathOperator{\Delt}{Q} %\mathbf{\Delta}}
\DeclareMathOperator{\Gam}{\mathbf{\Gamma}}
\DeclareMathOperator{\Gami}{\mathbf{\Gamma}^{-1}}
\DeclareMathOperator{\Sigb}{\mathbf{\Sigma}}


\newtheorem{Def}{Definition}
\newcommand\floor[1]{\lfloor#1\rfloor}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\floatname{algorithm}{Algorithm}


%%%%%%%% ALI ADDITIONS %%%%%%%%%%%%%%%%%%%%

\providecommand{\RR}{\Gamma} %real numbers
\newcommand{\Nat}{I\!\!N} %natural numbers

\newcommand{\cT}{\mathcal{T}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cK}{\mathcal{K}}

% \newcommand{\T}{\mathbf{T}}
% \newcommand{\X}{\mathbf{X}}
% \newcommand{\Y}{\mathbf{Y}}
% \newcommand{\W}{\mathbf{W}}
% \newcommand{\Z}{\mathbf{Z}}

\newcommand{\N}{\mathbb{N}}
\newcommand{\E}[2]{\mathbb{E}_{#1}\left[#2\right]}
\renewcommand{\P}[2]{P_{#1}\left[#2\right]}
\newcommand{\I}[2]{\mathbb{I}_{#1}\left\{#2\right\}}
% \newcommand{\R}{\mathbb{R}}

\newcommand{\indep}{\raisebox{0.05em}{\rotatebox[origin=c]{90}{$\models \;$}}}
\newcommand{\up}[1]{^{(#1)}}

\newcommand{\TE}{\text{TE}}
\newcommand{\ME}{\text{ME}}
\newcommand{\LE}{\mathsf{LE}}
\newcommand{\LLE}{\text{LLE}}
\newcommand{\FTE}{\text{FTE}}
\newcommand{\BTE}{\text{BTE}}
% \newcommand{\abs}[1]{\left\lvert #1 \right\rvert}


\newtheorem{application}{Application}[section]

% \newcommand{\D}{\mathbf{S}}

% this is to suppress badness warnings
\pgfplotsset{compat=1.17}
\hfuzz=100pt
\global\hbadness=10001
\global\vbadness=10001

